Piecewise Polynomial Regression of Tame Functions via Integer Programming

Tame functions are a class of nonsmooth, nonconvex functions, which feature in a wide range of applications: functions encountered in the training of deep neural networks with all common activations, value functions of mixed-integer programs, or wave functions of small molecules. We consider approximating tame functions with piecewise polynomial functions. We bound the quality of approximation of a tame function by a piecewise polynomial function with a given number of segments on any full-dimensional cube. We also present the first mixed-integer programming formulation of piecewise polynomial regression. Together, these can be used to estimate tame functions. We demonstrate promising computational results.

==> appx_neuripschecklist.tex <==
%%% BEGIN INSTRUCTIONS %%%


%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: We have theorems, proofs, and experiments to support the claims. 

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: We explain our Main result is limited to cubic domains (Remarik 1) and regular partitioning of the domain (Remark 2). We also discuss the run-time in Conclusions. 

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide proofs in the supplemental material, together with a short proof sketch to in the main body of the paper.

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The complete source code is provided in the Supplementary material and will be open-sourced upon acceptance. 


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer:\answerYes{}
    \item[] Justification: The benchmark instances are provided in the Supplementary material and will be open-sourced upon acceptance. 

\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} %
    \item[] Justification: The experimental setting is presented in the body of the paper to a level of detail that is necessary to appreciate the results. The full details can be provided either with the code, in appendix and in the supplemental material.

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{}.
    \item[] Justification: We report results of a deterministic optimization method, which allows only for a small variability in the runtime. 

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{}.
    \item[] Justification: We have used only a single Lenovo Thinkpad laptop. 

\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes.
    \item[] Justification: 


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is theory of ML, without immediate broader impacts. Eventually, it may lead to exact methods for training deep learning, which could be more trustworthy than the present ones. 

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper poses no such risks.


\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite the authors of the original benchmarks in Section 5. 

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The benchmark instances are provided in the Supplementary material and will be open-sourced upon acceptance. 

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{} 

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} 
    
\end{enumerate}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_neurips"
%%% End:


==> appx_proofmain.tex <==
We recall \cref{th:main}:
\mainres*

\Cref{th:main} will follow from a slightly more general result.
Let $\piecePolySpaceCuts(\appDom)$ denote the set of piecewise polynomial functions such that
\emph{(i)} the cells of the function form a hierarchical partition of $\appDom$ of depth $\nCuts$, and \emph{(ii)} the polynomial on each piece has degree at most $\polyDeg$.
% with a hierarchical partition of depth $\nCuts$ (\ie{} the function modeled by the MIP with depth $D = \nCuts$).
This is exactly the class of piecewise polynomial functions modelled by the mixed-integer formulation of \cref{sec:mip-form}.
This result gives an upper bound on the approximation error of a tame function by polynomials in that function class.
% the best piecewise polynomial function such that \emph{(i)} the cells of the polynomial form a hierarchical partition of $\appDom$ of depth $\nCuts$, and \emph{(ii)} the polynomial on each piece has degree at most $\polyDeg$.
\begin{theorem}\label{th:appx}
  Consider a cubic set $\appDom$, a function $f:\appDom\to\bbR$, and a constant $K>0$ such that:
  \begin{itemize}
    \item $f$ is definable in an o-minimal structure, and
    \item $f$ is $K$-Lipschitz on $\appDom$: for all $x$, $y\in\appDom$, $|f(x) - f(y)| \le K \|x-y\|$.
  \end{itemize}
  Then $f$ is piecewise approximable by polynomials: for any integers $\nCuts\ge 1$, and $\polyDeg \ge \smoothDeg > 1$, there holds
  \begin{equation}
    \inf_{p \in \piecePolySpaceCuts(\appDom)} \| f - p\|_{\infty, \appDom} \le \max\left( \frac{\constalt_1}{\nCuts^{\smoothDeg} \polyDeg^{\smoothDeg-1}}, \frac{\constalt_2}{\nCuts}\right),
  \end{equation}
  where $\constalt_{1} = \ndim^{\smoothDeg} \diam(\appDom)^\smoothDeg \const_{\ndim,\smoothDeg} \sum_{j=1}^{\ndim} \left \| \frac{\partial^{\smoothDeg}f}{\partial x_j^{\smoothDeg}} \right\|_{\infty,\diff(f)}$, $\constalt_{2} = \ndim K \diam(\appDom)$, and $\const_{d,r}$ is a constant that depends only on $d$ and $r$.
\end{theorem}

%\gbcomment{There should be some dimensionality curse in the second term of (24): a $\sqrt{d}$ term.}

% \gbcomment{def of hierarchical partition. Adapt proof.}

Before proceeding to the proof of \cref{th:appx}, we recall a result from approximation of $\C^{\smoothDeg}$ functions on a cube mentionned in \citet{plesniakMultivariateJacksonInequality2009}.
\begin{proposition}[Multivariate Jackson theorem]%
  \label{prop:jackson}
  Let $X$ be a compact cube in $\bbR^{\ndim}$, $f:\,X\to\bbR$ a $\mathcal{C}^{\smoothDeg}(X)$ function, and $\polyDeg\ge\smoothDeg$ two integers. Then
  there exists a constant $\const_{\ndim,\smoothDeg}$ depending only on $\ndim$, and $\smoothDeg$ such that:
  \begin{equation}
    \inf_{p\in \polySpace(X)} \|f - p\|_{\infty, X} \leq \rCube(X)^{\smoothDeg} \frac{\const_{\ndim,\smoothDeg}}{\polyDeg^{\smoothDeg-1}}\sum_{j=1}^{\ndim} \left\| \frac{\partial^{\smoothDeg}f}{\partial x_{j}^{\smoothDeg}} \right\|_{\infty, X},
  \end{equation}
  where $\rCube(X)$ denotes the edge length of $X$.
\end{proposition}
\begin{proof}[Proof of \cref{prop:jackson}]
    This result is obtained by reproducing the steps of Proposition 2.4 of \citet{plesniakExtensionPolynomialApproximation1994}, specializing to a cube which edge have same length $\rCube(X)$, and tracking the dependency in the size of the cube when combining Theorem 2.1 and Lemma 2.2 in \citet{plesniakExtensionPolynomialApproximation1994}.
\end{proof}
\begin{remark}
    We are not aware of a similar results in prominent approximation theory literature \cite{ditzian2012moduli,totik2020polynomial,dai2023polynomial} that propose an approximation result on a cubic domain, in which the constant $\const$ is independent of the geometry of the domain.
    This last point is essential for our purposes, since this result will be applied to small domains the size of which depends on parameters $\polyDeg$ and $\nPieces$ of \Cref{th:main}.
    % Having a constant $\const$ in the proof that does not depend on the geometry of the approximation domain $X$ is essential for our purposes.
\end{remark}

We now proceed with the proof of \cref{th:appx}.
\begin{proof}[Proof of \cref{th:appx}]
  % Consider the smallest hypercube enclosing the approximation set $\appDom$.
  Consider the set $\cubes$ of closed cubes obtained by regularly slicing the approximation domain $\nslice \eqdef \lfloor \nCuts / \ndim \rfloor + 1$ times along each cartesian axis.
  % Its radius is $\diam(\appDom)$, the diameter of $\appDom$.
  The domain $\appDom$ is thus split in $\nPieces = \nslice^{\ndim}$ pieces, each of which is a cube of edge length $\diam(\appDom) / \nslice$.
  Consider the set $\mathcal{P}_{\nslice}$ of functions from $\appDom$ to $\bbR$ such that the restriction to any cube of $\cubes$ is a polynomial of degree up to $\polyDeg$.
  Since $\mathcal{P}_{\nslice} \subset \piecePolySpaceCuts$, there holds
  \begin{equation}
    \inf_{p\in\piecePolySpaceCuts} \|f - p\|_{\infty, \appDom} \le \inf_{p \in \mathcal{P}_{\nslice}} \|f - p\|_{\infty, \appDom}.
  \end{equation}

  Since $f$ is definable, \cref{prop:celldecomp} yields a finite collection $\Mcol$ of cells $\M\subset\bbR^{\ndim}$, such that each cell is open, definable, full-dimensional, any two cells are disjoint, and the union of the closure of the cells is $\appDom$.
  Then, define the following subsets of $\cubes$:
  \begin{equation}
    \cubesU = \{ c \in \cubes : \exists \M \in \Mcol, c \subset \M \}, \qquad \cubesV = \cubes \setminus \cubesU.
  \end{equation}
  % $\cubesU$ as the set of cubes of $\cubes$ such that is either contained in the closure of an element of $\Mcol$.
  % define the partition of $\cubes$ in $\cubesU$ and $\cubesV$
  % Consider the subset $\cubesU$ of $\cubes$ that contains all the cubes that are contained in the closure of a full-dimensional cell.
  % Denote $\cubesV$ the set of all the cubes that are not contained in the closure of a full-dimensional strata.
  We have the following:
  \begin{align}
    \inf_{p \in \mathcal{P}_{\nslice}} \|f - p\|_{\infty, \appDom} &= \inf_{p\in\mathcal{P}_{\nslice}} \max\left(\max_{c \in \cubesU} \| f - p \|_{\infty, c}, \max_{c \in \cubesV} \| f - p \|_{\infty, c}\right) \\
                                          &= \max\left(\max_{c \in \cubesU} \inf_{p \in \polySpace(c)} \| f - p \|_{\infty, c}, \max_{c \in \cubesV} \inf_{p \in \polySpace(c)} \| f - p \|_{\infty, c}\right).
  \end{align}
  The first equality follows from the definition of the infinity norm and that the union of the cubes in $\cubesU$ and $\cubesV$ is $\appDom$.
  The second equality follow from the independence of the expression of any $p \in \mathcal{P}_{\nslice}$ on any two distinct cubes of $\cubes$.

  Let $c$ denote a cube in $\cubesU$.
  Since $c$ is contained in a cell $\M$ on which $f$ is $\C^{\smoothDeg}$, the restriction of $f$ to $c$ is $\C^{r}$.
  % [
  % $f$ is $\C^{r}$ on $\M_{c}$.
  % $f$ admits a natural expansion to $\cl(\M_{c})$ that is continuous. [Is it $\C^{r}$].
  % Does $f$ admits a $\C^{r}$ expansion from $\M_{c}$ to $\cl(\M_{c})$? If so, any will do.
  % ]
  % \gbcomment{
  %   Handle:
  %   [$f$ is $\C^{r}$ on the open set $\M$. What about on $\cl(\M)$?]
  %   [($\polyDeg > r-1$)]
  % }
  Therefore, \cref{prop:jackson} applies and yield
  \begin{equation}\label{eq:boundint}
    \inf_{p \in \polySpace(c)} \| f - p \|_{\infty, c} \le \left(\frac{\rCube(\appDom)}{\nslice}\right)^{\smoothDeg} \frac{\const_{\ndim,\smoothDeg}}{\polyDeg^{\smoothDeg-1}}\sum_{j=1}^{\ndim} \left\| \frac{\partial^{\smoothDeg}f}{\partial x_j^{\smoothDeg}}\right\|_{\infty, c}%\sup_{x\in c}\left|\frac{\partial^{\smoothDeg}f}{\partial x_j^{\smoothDeg}}(x)\right|.
  \end{equation}
  for some constant $\const_{\ndim,\smoothDeg}$ depending only on $\ndim$ and $\smoothDeg$.

  Let $c$ denote a cube in $\cubesV$, and $x_{0}$ denote an arbitray point in $c$.
  Since $f$ is $K$-Lipschitz, for any $x\in c$,
  \begin{equation}
    | f(x) - f(x_{0}) | \le K \|x - x_{0}\|.
  \end{equation}
  Thus,
  \begin{equation}\label{eq:boundbound}
    \| f(x) - f(x_{0}) \|_{\infty, c} \le K \sup_{x\in c}\|x - x_{0}\| \le K \diam(c) = K \diam(\appDom) \nslice^{-1}.
  \end{equation}

  Combining the two bounds \eqref{eq:boundint} and \eqref{eq:boundbound}, and using $\nslice = \lfloor \nCuts / \ndim \rfloor + 1 \ge \nCuts / \ndim$ yields
  \begin{align}
    \inf_{p \in \piecePolySpaceCuts(\appDom)} \| f - p\|_{\infty, \appDom} &\le \max \left(\frac{\diam(\appDom)^\smoothDeg}{\nslice^{\smoothDeg}}\frac{\const_{\ndim,\smoothDeg}}{\polyDeg^{\smoothDeg-1}} \sum_{j=1}^{\ndim} \left \| \frac{\partial^{\smoothDeg}f}{\partial x_j^{\smoothDeg}} \right\|_{\infty,\diff(f)}, \frac{K \diam(\appDom)}{\nslice} \right) \\
    & \le \max \left(\frac{\ndim^{\smoothDeg}\diam(\appDom)^\smoothDeg}{\nCuts^{\smoothDeg}}\frac{\const_{\ndim,\smoothDeg}}{\polyDeg^{\smoothDeg-1}} \sum_{j=1}^{\ndim} \left \| \frac{\partial^{\smoothDeg}f}{\partial x_j^{\smoothDeg}} \right\|_{\infty,\diff(f)}, \frac{\ndim K \diam(\appDom)}{\nCuts} \right) \\
    % & = \max\left( \bigoh\left(\frac{1}{\nPieces \polyDeg^{\smoothDeg-1}}\right), \bigoh\left(\frac{1}{\nPieces^{1/\ndim}}\right) \right). \\
      & = \max\left( \frac{\constalt_1}{\nCuts^{\smoothDeg} \polyDeg^{\smoothDeg-1}}, \frac{\constalt_2}{\nCuts}\right).
  \end{align}
  where $\constalt_{1} = \ndim^{\smoothDeg} \diam(\appDom)^\smoothDeg \const_{\ndim,\smoothDeg} \sum_{j=1}^{\ndim} \left \| \frac{\partial^{\smoothDeg}f}{\partial x_j^{\smoothDeg}} \right\|_{\infty,\diff(f)}$ and $\constalt_{2} = \ndim K \diam(\appDom)$.
  % where $\const = \max_{c \in \cubesU} \const_{c}$.
  % \gbcomment{Fix rad vs diam}
  % \gbcomment{Adapt main theorem statement to this.}
\end{proof}

We can now deduce the result of \cref{th:main}.
\begin{proof}[Proof of \cref{th:main}]
  Consider a number of pieces $\nPieces$ and the highest number of cuts that allow splitting a cube in $\bbR^{\ndim}$ in $\nPieces$, that is the highest $\nCuts$ such that $\nPieces \ge (\lfloor \nCuts / \ndim \rfloor + 1)^{\ndim}$.
  The bound of \cref{th:appx} applies to this situation and yields
  \begin{equation}\label{eq:thm1Proof}
    \inf_{p \in \piecePolySpace[\nslice^{\ndim}](\appDom)} \| f - p\|_{\infty, \appDom} \le \max \left(\frac{\diam(\appDom)^\smoothDeg}{\nPieces^{\frac{\smoothDeg}{\ndim}}}\frac{\const_{\ndim,\smoothDeg}}{\polyDeg^{\smoothDeg-1}} \sum_{j=1}^{\ndim} \left \| \frac{\partial^{\smoothDeg}f}{\partial x_j^{\smoothDeg}} \right\|_{\infty,\diff(f)}, \frac{K \diam(\appDom)}{\nPieces^{1/\ndim}} \right),
    % & = \max\left( \bigoh\left(\frac{1}{\nPieces \polyDeg^{\smoothDeg-1}}\right), \bigoh\left(\frac{1}{\nPieces^{1/\ndim}}\right) \right). \\
      % & = \max\left( \frac{\const_1}{\nPieces \polyDeg^{\smoothDeg-1}}, \frac{\const_2}{\lfloor \nPieces^{1/\ndim} \rfloor}\right).
  \end{equation}
  since $\nPieces^{1/\ndim} \ge \nCuts / \ndim$, which is the claimed bound.
  % where $\const_{1} = \diam(\appDom)^\ndim \const_{\ndim,\smoothDeg} \sum_{j=1}^{\ndim} \left \| \frac{\partial^{\smoothDeg}f}{\partial x_j^{\smoothDeg}} \right\|_{\infty,\diff(f)}$ and $\const_{2} = K \diam(\appDom)$.
\end{proof}

% \textcolor{red}{TODO: Main issue is how to deal with the openess of the cells/stratifications. The SW or Jackson theorems are for closed sets. \cite{aschenbrenner2019whitney} could have some answers, see also below.}

% \textcolor{red}{TODO (Johannes): Work this theorem out, what happens with Jackson when the cells are open boxes and not closed as in the ordinary Jackson? Because this is the case for the cell decomposition. IT DOES NOT WORK IN GENERAL!!! What is the rate of convergence? }

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_icml"
%%% End:

